Risk-Driven Design of Perception Systems

Modern autonomous systems rely on perception modules to process complex sensor measurements into state estimates. These estimates are then passed to a controller, which uses them to make safety-critical decisions. It is therefore important that we design perception systems to minimize errors that reduce the overall safety of the system. We develop a risk-driven approach to designing perception systems that accounts for the effect of perceptual errors on the performance of the fully-integrated, closed-loop system. We formulate a risk function to quantify the effect of a given perceptual error on overall safety, and show how we can use it to design safer perception systems by including a risk-dependent term in the loss function and generating training data in risk-sensitive regions. We evaluate our techniques on a realistic vision-based aircraft detect and avoid application and show that risk-driven design reduces collision risk by 37% over a baseline system.

==> altitude_risk_profile.tex <==

\nextgroupplot [
  height = {3cm},
  ylabel = {Altitude (m)},
  xmin = {0.0},
  xmax = {40.0},
  ymax = {1370.0},
  ytick = {1300, 1340},
  xticklabels={,},
  ymin = {1280.0},
  width = {10cm},
  xmajorticks=false,
  ytick pos=left,
  legend pos=south west,
  legend columns=-1,
  legend style={font=\tiny}
]

\addplot+[
  mark = {none},
  thick, red
] coordinates {
  (0.0, 1356.3454033744606)
  (1.0, 1356.3454033744606)
  (2.0, 1356.3454033744606)
  (3.0, 1356.3454033744606)
  (4.0, 1356.3454033744606)
  (5.0, 1356.3454033744606)
  (6.0, 1356.3454033744606)
  (7.0, 1356.3454033744606)
  (8.0, 1356.3454033744606)
  (9.0, 1356.3454033744606)
  (10.0, 1356.3454033744606)
  (11.0, 1356.3454033744606)
  (12.0, 1356.3454033744606)
  (13.0, 1356.3454033744606)
  (14.0, 1356.3454033744606)
  (15.0, 1356.3454033744606)
  (16.0, 1356.3454033744606)
  (17.0, 1356.8454033744606)
  (18.0, 1356.8454033744606)
  (19.0, 1356.8454033744606)
  (20.0, 1357.3454033744606)
  (21.0, 1357.3454033744606)
  (22.0, 1357.3454033744606)
  (23.0, 1356.8454033744606)
  (24.0, 1356.8454033744606)
  (25.0, 1356.8454033744606)
  (26.0, 1356.8454033744606)
  (27.0, 1356.8454033744606)
  (28.0, 1356.8454033744606)
  (29.0, 1356.8454033744606)
  (30.0, 1357.3454033744606)
  (31.0, 1357.3454033744606)
  (32.0, 1357.3454033744606)
  (33.0, 1357.3454033744606)
  (34.0, 1357.3454033744606)
  (35.0, 1357.3454033744606)
  (36.0, 1357.8454033744606)
  (37.0, 1357.8454033744606)
  (38.0, 1357.8454033744606)
  (39.0, 1357.8454033744606)
  (40.0, 1357.8454033744606)
  (41.0, 1357.8454033744606)
  (42.0, 1357.8454033744606)
  (43.0, 1357.8454033744606)
  (44.0, 1357.8454033744606)
  (45.0, 1358.3454033744606)
  (46.0, 1358.3454033744606)
  (47.0, 1358.3454033744606)
  (48.0, 1358.8454033744606)
  (49.0, 1358.8454033744606)
};

\addplot+[
  mark = {none},
  thick, pastelPurple
] coordinates {
  (0.0, 1325.0257792707625)
  (1.0, 1325.0257792707625)
  (2.0, 1325.5257792707625)
  (3.0, 1325.5257792707625)
  (4.0, 1325.5257792707625)
  (5.0, 1325.5257792707625)
  (6.0, 1325.5257792707625)
  (7.0, 1325.0257792707625)
  (8.0, 1325.0257792707625)
  (9.0, 1325.0257792707625)
  (10.0, 1325.5257792707625)
  (11.0, 1325.5257792707625)
  (12.0, 1325.5257792707625)
  (13.0, 1325.5257792707625)
  (14.0, 1325.5257792707625)
  (15.0, 1326.0257792707625)
  (16.0, 1325.5257792707625)
  (17.0, 1325.5257792707625)
  (18.0, 1325.5257792707625)
  (19.0, 1326.0257792707625)
  (20.0, 1325.5257792707625)
  (21.0, 1325.5257792707625)
  (22.0, 1326.0257792707625)
  (23.0, 1326.0257792707625)
  (24.0, 1326.0257792707625)
  (25.0, 1325.5257792707625)
  (26.0, 1324.5257792707625)
  (27.0, 1322.5257792707625)
  (28.0, 1321.5257792707625)
  (29.0, 1319.5257792707625)
  (30.0, 1318.5257792707625)
  (31.0, 1316.5257792707625)
  (32.0, 1315.5257792707625)
  (33.0, 1313.5257792707625)
  (34.0, 1311.0257792707625)
  (35.0, 1307.5257792707625)
  (36.0, 1302.5257792707625)
  (37.0, 1296.5257792707625)
  (38.0, 1291.5257792707625)
  (39.0, 1287.5257792707625)
  (40.0, 1285.0257792707625)
  (41.0, 1283.5257792707625)
  (42.0, 1283.0257792707625)
  (43.0, 1283.0257792707625)
  (44.0, 1283.0257792707625)
  (45.0, 1283.0257792707625)
  (46.0, 1283.5257792707625)
  (47.0, 1283.5257792707625)
  (48.0, 1283.5257792707625)
  (49.0, 1283.5257792707625)
};

\addplot+[
  mark = {none},
  thick, gray
] coordinates {
  (0.0, 1325.0257792707625)
  (1.0, 1325.0257792707625)
  (2.0, 1325.5257792707625)
  (3.0, 1325.5257792707625)
  (4.0, 1325.5257792707625)
  (5.0, 1325.5257792707625)
  (6.0, 1325.5257792707625)
  (7.0, 1325.0257792707625)
  (8.0, 1325.0257792707625)
  (9.0, 1325.0257792707625)
  (10.0, 1325.5257792707625)
  (11.0, 1325.5257792707625)
  (12.0, 1325.5257792707625)
  (13.0, 1325.5257792707625)
  (14.0, 1325.5257792707625)
  (15.0, 1326.0257792707625)
  (16.0, 1325.5257792707625)
  (17.0, 1325.5257792707625)
  (18.0, 1325.5257792707625)
  (19.0, 1326.0257792707625)
  (20.0, 1325.5257792707625)
  (21.0, 1325.5257792707625)
  (22.0, 1326.0257792707625)
  (23.0, 1326.0257792707625)
  (24.0, 1326.0257792707625)
  (25.0, 1326.5257792707625)
  (26.0, 1327.0257792707625)
  (27.0, 1326.5257792707625)
  (28.0, 1326.5257792707625)
  (29.0, 1326.5257792707625)
  (30.0, 1326.5257792707625)
  (31.0, 1325.5257792707625)
  (32.0, 1325.5257792707625)
  (33.0, 1325.5257792707625)
  (34.0, 1326.0257792707625)
  (35.0, 1325.5257792707625)
  (36.0, 1323.5257792707625)
  (37.0, 1320.5257792707625)
  (38.0, 1316.5257792707625)
  (39.0, 1313.5257792707625)
  (40.0, 1312.0257792707625)
  (41.0, 1311.5257792707625)
  (42.0, 1311.5257792707625)
  (43.0, 1311.5257792707625)
  (44.0, 1311.5257792707625)
  (45.0, 1311.5257792707625)
  (46.0, 1312.0257792707625)
  (47.0, 1312.0257792707625)
  (48.0, 1312.0257792707625)
  (49.0, 1312.0257792707625)
};

\addplot+[
  draw = none,
  mark = {*},
  mark options = {fill=gray, draw=gray}
] coordinates {
  (25.0, 1326.5257792707625)
  (29.0, 1326.5257792707625)
  (33.0, 1325.5257792707625)
  (34.0, 1326.0257792707625)
  (35.0, 1325.5257792707625)
  (36.0, 1323.5257792707625)
};

\addplot+[
  draw = none,
  mark = {*},
  mark options = {fill=pastelPurple, draw=pastelPurple}
] coordinates {
  (23.0, 1326.0257792707625)
  (24.0, 1326.0257792707625)
  (25.0, 1325.5257792707625)
  (27.0, 1322.5257792707625)
  (29.0, 1319.5257792707625)
  (31.0, 1316.5257792707625)
  (32.0, 1315.5257792707625)
  (33.0, 1313.5257792707625)
  (34.0, 1311.0257792707625)
  (35.0, 1307.5257792707625)
};

\addplot+[
  mark = {none},
  black, dashed,
  opacity = 0.5
] coordinates {
  (23, 1280)
  (23, 1370)
};

\addplot+[
  mark = {none},
  black, dashed,
  opacity = 0.5
] coordinates {
  (25, 1280)
  (25, 1370)
};

\addplot+[
  mark = {none},
  black, dashed,
  opacity = 0.5
] coordinates {
  (31, 1280)
  (31, 1370)
};

\addplot+[
  mark = {none},
  black, dashed,
  opacity = 0.5
] coordinates {
  (35, 1280)
  (35, 1370)
};
%\legend{intruder, baseline, risk sensitive};


\nextgroupplot [
  height = {3cm},
  ylabel = {Risk},
  xmin = {0.0},
  xmax = {40.0},
  ymax = {120.0},
  ytick = {80, 100},
  xlabel = {Time (s)},
  ylabel style = {yshift = 0.25cm},
  ymin = {70.0},
  width = {10cm},
  ytick pos=left,
  xtick pos=left
]

\addplot+[
  mark = {none},
  thick, pastelPurple
] coordinates {
  (0.0, 89.48735726433932)
  (1.0, 89.79573304868279)
  (2.0, 89.77922726118277)
  (3.0, 89.77381734738847)
  (4.0, 89.76841598921801)
  (5.0, 89.76301772181199)
  (6.0, 89.49502388832549)
  (7.0, 89.44709224623585)
  (8.0, 89.45011124646122)
  (9.0, 89.77368982852055)
  (10.0, 89.77290713323568)
  (11.0, 89.78867009329207)
  (12.0, 89.80931673877188)
  (13.0, 89.83318939191467)
  (14.0, 90.18174814641534)
  (15.0, 89.9329663002657)
  (16.0, 89.66664495203044)
  (17.0, 89.68732331485617)
  (18.0, 90.11920221845187)
  (19.0, 89.67978262632207)
  (20.0, 89.79108697025418)
  (21.0, 90.45346382651495)
  (22.0, 91.27556001269943)
  (23.0, 89.69067554048544)
  (24.0, 87.74981513078754)
  (25.0, 85.23584008322187)
  (26.0, 90.1254735379376)
  (27.0, 85.35867955659772)
  (28.0, 91.55881982740794)
  (29.0, 84.96917890417683)
  (30.0, 94.31396675166425)
  (31.0, 92.15289277137876)
  (32.0, 90.13739599900973)
  (33.0, 90.6535878440617)
  (34.0, 89.84816963909009)
  (35.0, 87.4582641211309)
  (36.0, 88.17295349335808)
  (37.0, 88.16124446130358)
  (38.0, 83.68037589630184)
  (39.0, 79.68037589630184)
  (40.0, 74.16014274057646)
  (41.0, 74.2375318218966)
  (42.0, 74.2657889108005)
  (43.0, 74.2657889108005)
  (44.0, 73.79527230094644)
  (45.0, 74.05164586969343)
  (46.0, 74.2657889108005)
  (47.0, 73.79527230094644)
  (48.0, 73.82545631819121)
  (49.0, 74.27783542119563)
};


\addplot+[
  mark = {none},
  thick, gray
] coordinates {
  (0.0, 89.48735726433932)
  (1.0, 89.79573304868279)
  (2.0, 89.77922726118277)
  (3.0, 89.77381734738847)
  (4.0, 89.76841598921801)
  (5.0, 89.76301772181199)
  (6.0, 89.49502388832549)
  (7.0, 89.44709224623585)
  (8.0, 89.45011124646122)
  (9.0, 89.77368982852055)
  (10.0, 89.77290713323568)
  (11.0, 89.78867009329207)
  (12.0, 89.80931673877188)
  (13.0, 89.83318939191467)
  (14.0, 90.18174814641534)
  (15.0, 89.9329663002657)
  (16.0, 89.66664495203044)
  (17.0, 89.68732331485617)
  (18.0, 90.11920221845187)
  (19.0, 89.67978262632207)
  (20.0, 89.79108697025418)
  (21.0, 90.45346382651495)
  (22.0, 91.27556001269943)
  (23.0, 91.9577165487872)
  (24.0, 93.41523708075961)
  (25.0, 93.56249214243519)
  (26.0, 96.82535442980249)
  (27.0, 99.2717835176012)
  (28.0, 102.15784556824939)
  (29.0, 97.15098415829578)
  (30.0, 107.18345121032908)
  (31.0, 110.29792463181838)
  (32.0, 113.135917044591)
  (33.0, 114.63215476624399)
  (34.0, 114.10470837124402)
  (35.0, 111.75338428976595)
  (36.0, 112.27443658376667)
  (37.0, 112.26507061748184)
  (38.0, 108.68037589630181)
  (39.0, 105.68037589630181)
  (40.0, 82.19435830833356)
  (41.0, 82.07315424859584)
  (42.0, 82.07315424859584)
  (43.0, 82.07315424859584)
  (44.0, 82.01262400617932)
  (45.0, 82.12131798722012)
  (46.0, 82.07315424859584)
  (47.0, 82.01262400617932)
  (48.0, 81.88250374766298)
  (49.0, 82.36013222677725)
};

\addplot+[
  draw = none,
  mark = {*},
  mark options = {fill=gray, draw=gray}
] coordinates {
  (25.0, 93.56249214243519)
  (29.0, 97.15098415829578)
  (33.0, 114.63215476624399)
  (34.0, 114.10470837124402)
  (35.0, 111.75338428976595)
  (36.0, 112.27443658376667)
};

\addplot+[
  draw = none,
  mark = {*},
  mark options = {fill=pastelPurple, draw=pastelPurple}
] coordinates {
  (23.0, 89.69067554048544)
  (24.0, 87.74981513078754)
  (25.0, 85.23584008322187)
  (27.0, 85.35867955659772)
  (29.0, 84.96917890417683)
  (31.0, 92.15289277137876)
  (32.0, 90.13739599900973)
  (33.0, 90.6535878440617)
  (34.0, 89.84816963909009)
  (35.0, 87.4582641211309)
};

\addplot+[
  mark = {none},
  black, dashed,
  opacity = 0.5
] coordinates {
  (23, 70)
  (23, 120)
};

\addplot+[
  mark = {none},
  black, dashed,
  opacity = 0.5
] coordinates {
  (25, 70)
  (25, 120)
};

\addplot+[
  mark = {none},
  black, dashed,
  opacity = 0.5
] coordinates {
  (31, 70)
  (31, 120)
};

\addplot+[
  mark = {none},
  black, dashed,
  opacity = 0.5
] coordinates {
  (35, 70)
  (35, 120)
};


==> ground_track.tex <==

\addplot+[
  mark = {none},
  thick, gray
] coordinates {
  (1002.3609512491221, 155.21153381044792)
  (999.8455360334633, 203.68131327469004)
  (997.3301208178054, 252.15109273893185)
  (994.8147056021471, 300.62087220317375)
  (992.2992903864888, 349.0906516674158)
  (989.7838751708305, 397.5604311316577)
  (987.2684599551721, 446.0302105958998)
  (984.7530447395143, 494.49999006014167)
  (982.2376295238555, 542.9697695243835)
  (979.7222143081976, 591.4395489886258)
  (977.2067990925393, 639.9093284528675)
  (974.691383876881, 688.3791079171096)
  (972.1759686612227, 736.8488873813515)
  (969.6605534455643, 785.3186668455934)
  (967.1451382299065, 833.7884463098356)
  (964.6297230142482, 882.2582257740773)
  (962.1143077985898, 930.7280052383189)
  (959.5988925829315, 979.197784702561)
  (957.0834773672732, 1027.667564166803)
  (954.5680621516153, 1076.137343631045)
  (952.0526469359565, 1124.6071230952869)
  (949.5372317202987, 1173.076902559529)
  (947.0218165046404, 1221.5466820237707)
  (944.506401288982, 1270.0164614880127)
  (941.9909860733237, 1318.4862409522548)
  (939.4755708576654, 1366.956020416497)
  (936.9601556420075, 1415.4257998807386)
  (934.4447404263492, 1463.8955793449807)
  (931.9293252106904, 1512.3653588092225)
  (929.4139099950326, 1560.8351382734645)
  (926.8984947793742, 1609.3049177377065)
  (924.3830795637159, 1657.7746972019486)
  (921.8676643480576, 1706.2444766661904)
  (919.3522491323997, 1754.7142561304324)
  (916.8368339167414, 1803.1840355946742)
  (914.3214187010826, 1851.6538150589163)
  (911.8060034854248, 1900.1235945231583)
  (909.2905882697664, 1948.5933739874001)
  (906.7751730541086, 1997.0631534516422)
  (904.2597578384498, 2045.5329329158842)
  (901.7443426227915, 2094.002712380126)
};

\addplot+[
  mark = {none},
  thick, red
] coordinates {
  (255.43001759246818, 3690.742801935951)
  (272.8341360188433, 3646.611921952227)
  (290.23825444521754, 3602.481041968504)
  (307.64237287159267, 3558.350161984781)
  (325.0464912979669, 3514.219282001058)
  (342.45060972434203, 3470.0884020173344)
  (359.85472815071626, 3425.9575220336114)
  (377.2588465770914, 3381.8266420498876)
  (394.6629650034665, 3337.6957620661647)
  (412.06708342984075, 3293.564882082441)
  (429.4712018562159, 3249.434002098718)
  (446.8753202825901, 3205.303122114995)
  (464.27943870896524, 3161.172242131271)
  (481.6835571353404, 3117.0413621475477)
  (499.0876755617146, 3072.910482163825)
  (516.4917939880897, 3028.779602180102)
  (533.8959124144649, 2984.648722196378)
  (551.3000308408386, 2940.517842212655)
  (568.7041492672138, 2896.386962228931)
  (586.1082676935885, 2852.2560822452083)
  (603.5123861199636, 2808.1252022614854)
  (620.9165045463383, 2763.994322277762)
  (638.3206229727134, 2719.8634422940386)
  (655.7247413990881, 2675.732562310315)
  (673.1288598254628, 2631.601682326592)
  (690.5329782518379, 2587.4708023428684)
  (707.9370966782121, 2543.3399223591455)
  (725.3412151045868, 2499.209042375422)
  (742.745333530962, 2455.078162391699)
  (760.1494519573366, 2410.9472824079758)
  (777.5535703837113, 2366.8164024242524)
  (794.957688810086, 2322.685522440529)
  (812.3618072364611, 2278.5546424568056)
  (829.7659256628358, 2234.423762473082)
  (847.17004408921, 2190.2928824893593)
  (864.5741625155852, 2146.162002505636)
  (881.9782809419598, 2102.0311225219125)
  (899.3823993683345, 2057.9002425381896)
  (916.7865177947097, 2013.7693625544662)
  (934.1906362210843, 1969.6384825707428)
  (951.594754647459, 1925.5076025870194)
};

